A Query-Driven Decision Procedure for Distributed Autoepistemic Logic with Inductive Definitions

Distributed Autoepistemic Logic with Inductive Definitions (dAEL(ID)) is a recently proposed non-monotonic logic for says-based access control. We define a query-driven decision procedure for dAEL(ID) that is implemented in the knowledge-base system IDP. The decision procedure is designed in such a way that it allows one to determine access rights while avoiding redundant information flow between principals in order to enhance security and reduce privacy concerns. Given that the decision procedure has in the worst case an exponential runtime, it is to be regarded as a proof of concept that increases our understanding of dAEL(ID), rather than being deployed for an access control system.

==> conclusion.tex <==
\section{Conclusions}\label{sec:conc}

In this paper we have defined and studied \emph{Distributed Access Control Logic} (\DACL), a non-monotonic \say-based access control logic. The non-monotonicity of \DACL makes it possible to model access denials more straightforwardly than in state-of-the-art access control logics. We have presented principled motivations for the features of \DACL, especially the usage of autoepistemic logic with the well-founded semantics and the inclusion of inductive definitions, and have illustrated the practical relevance of these principled motivations with reference to access control application scenarios. We have defined a query-based decision procedure for \DACL, which avoids redundant information flow between principals in order to reduce privacy concerns.

==> unconstrained.tex <==
\section{Introduction}


In recent years many logics have been proposed to specify access control frameworks. Such logics, used to represent and reason about policies in access control, are based on a small number of primitive notions. Barker \cite{Barker:2009:NAC:1542207.1542238} proposes a meta-model capable of dealing with the dynamic changes of the requirements. Barker's proposal defines the primitive building blocks that are common to access control.


%We extend propositional logic with \emph{says} operator. This multi-modal logic is the basic building block that allows the definition of policies. \

We define a new logic that generalises Barker's meta-model and has semantics more suitable for the intended application. It is capable of specifying access control policies. Making use of the model expansion inference of IDP, this declarative policy specification becomes an executable program which can function as a reference monitor for handling access requests. We also illustrate how the IDP implementation can help to shed light on the formal properties (invariants) that need to be satisfied in access control systems. Thus, allowing to reason about such properties and access control systems generated by combining different properties.

The IDP framework is not query driven. To be able to perform queries, we implement a meta-theoretical querying mechanism.


This modular approach allow users to write their own policies in modal propositional logic language referring to other users' policies using the says modality.


Formulas from the propositional says based logic will be the objects that we will reason and talk about and we treat them as first class citizen. We define a translation mechanism to include the says logic into IDP.

%In a distributed computing context principals often have to reason about authorisations with incomplete forms of information. To fill in the gaps in the principals' knowledge we allow principals to communicate. We implement a mechanism similar to remote predicate calls present in other systems like ...[DLV, Valerio].


\section{A Policy Specification Language}\label{sec:dacl}

\subsection{Definition}


In this section we present the ploicy specification language \DACL which allows to specify and reason about distributed access control policies. We consider a distributed access control model, where policy information is scattered among several principals. Principals can support policy statements and also rely on statements from other principals to make their assertions.

The \emph{\says} predicate represents the remote information contained in different theories belonging to other principals.

\DACL is an access control logic which extends propositional logic with a modality \emph{\says} indexed by a principal $A$ and enriched with inductive definitions. Intuitively the meaning of $A ~\says~ \varphi$ is ``$A$ supports $\varphi$''.


\subsubsection{\DACL Syntax} formulas, inductive definitions, theories, principals, modality, \ldots


We have four type of objects, \emph{principals}, \emph{inductive definitions}, \emph{theories} and a \emph{modality}.
%\DACL allows for inductive definitions



%The syntax of \DACL is defined by

\begin{definition}  Formulae of \DACL is defined by the following EBNF rule:
 \[\varphi ::= p \mid \neg \varphi \mid (\varphi \land \varphi) \mid A ~\says~ \varphi \]
% \[\delta ::= p \leftarrow \varphi \mid \delta, p \leftarrow \varphi \]
% \[ T_A ::= \varphi \mid \{ \delta \} \mid T_A, \varphi \mid T_A, \{\delta \} \]
\end{definition}

\begin{definition}
We define a \DACL \emph{inductive definition} $\Delta$ to be a finite set of rules of the form $\{p \leftarrow \varphi\}$ where $p$ is a propositional variable and $\varphi$ is a \DACL formula.
\end{definition}

\begin{definition}
A \DACL \emph{theory} is a set that consists of \DACL formulae and \DACL inductive definitions.
\end{definition}
%This special says-predicate take as arguments the name (or address) of another principal\footnote{For simplicity we use the IP address of the nodes, representing the principals, and an specific port to establish the communication.} and a $\varphi$-term representing the formula we want to remotely query to the principal.


\subsection{Motivation}

\DACL includes a formal construct for inductive definitions. Inductive definitions are a common concept in all branches of mathematics. Below we give an example policy to show the usefulness of including inductive definitions in the policy specification language \DACL. Inductive definitions in D-ACL are intended to be understood in the same way as in the general purpose specification language \fodot of the \idp system [REF].

Because of their rule-based nature, formal inductive definitions also bear strong similarities in syntax and formal semantics with logic programming. A formal inductive definition could also be understood intuitively as a logic program which has arbitrary formulas in the body and which defines only a subset of the
predicates in terms of parameter predicates not defined in the definition.

\begin{example}
\[ \mathcal{T}_{A_1} = \left\{
\begin{split}
   & access\_A_1\_r \\
   & access\_A_2\_r  \leftarrow \bigvee\limits_{k = 1}^{n} (A_1 ~\says~ access\_A_k\_r \land A_k ~\says~ delegate\_to\_A_2)  \land \\
   &  ~~~~~~~~~~~~~~~~~~~~~~~~~ \neg \bigvee\limits_{i = 1}^{n} (A_1 ~\says~ access\_A_i\_r \land A_i ~\says~ revoke\_A_2) \\
   & ~~~~~~~~~~ \vdots \\
   & access\_A_n\_r  \leftarrow    \ldots
%   & access\_A_n\_r  \leftarrow \bigvee\limits_{k = 1}^{n} (A_1 ~\says~ access\_A_k\_r \land A_k ~\says~ delegate\_to\_A_n)  \land \\
%   &  ~~~~~~~~~~~~~~~~~~~~~~~~~ \neg \bigvee\limits_{i = 1}^{n} (A_1 ~\says~ access\_A_i\_r \land A_i ~\says~ revoke\_A_n) 
\end{split}
 \right\} \]
\end{example}


\section{\foid and the \idp-system}\label{sec:IDP}


\subsection{Why \idp?}



\subsection{The \idp System}

The aim in the development of the \idp-system is to integrate existing \emph{pure declarative KR-languages} with a \emph{knowledge base system} to implement reasoning for these languages.


We use the term  \foid for a family of extensions of first-order logic.
% \fodot is developed with the purpose to combine ideas from multiple domains of knowledge representation, logic programming and on monotonic reasoning in a conceptual clear manner.
The basis of this family of languages lies in first order (classical) logic, extended with new language constructs from the fields of logic programming, constraint programming and non-monotonic reasoning.


The \idp-system supports an \foid language, denoted by $\foid^{IDP}$. %In the context of this paper, the focus lies on \fodotidp, since this is the language used for the modelling of the revocation schemes further on.


This section provides a brief summary of the core of the \foid language, more details about the language can be found in \cite{WarrenBook/DeCatBBD14}.
We assume familiarity with basic concepts of classical logic and logic programming.
\foid extends first order logic with \emph{types, (partial) functions} and the key addition of \emph{inductive definitions}.


An \foid specification consists of a vocabulary, a theory and a (partial) structure.

A \emph{vocabulary} $\Sigma$ consists of a set of symbols, predicate symbols and function symbols. Symbols are types (sorts). Each predicate (function) symbol have an associated arity, the number of arguments they take. We sometimes use $P/n$ ($f/n$) to denote the predicate symbol $P$ (respectively function symbol $f$) with arity $n$. A function can be declared as \emph{partial}, indicating that for some inputs, the output can be undefined; otherwise it is \emph{total}.

A \emph{term} is a variable or an $n$-ary function symbol applied to $n$ terms. An \emph{atom} is an $n$-ary predicate symbol applied to $n$ terms. 
\emph{Formulas} are defined inductively: an atom is a formula; if $\varphi$ and $\varphi^\prime$ are formulas, then $\neg \varphi$, $\varphi \land \varphi^\prime$, $\varphi \lor \varphi^\prime$, $\forall x : \varphi$ and $\exists x : \varphi$ are also formulas. The expressions $\varphi \Rightarrow \varphi^\prime$, $\varphi \Leftarrow \varphi^\prime$ and $\varphi \Leftrightarrow \varphi^\prime$ are defined as usual.
A \emph{constant} can be interpreted as a $0-$\emph{ary} total function symbol.

A \emph{literal} $l$ is an atom $a$ or its negation $\neg a$. A \emph{sentence} is a formula without free (unquantified) variables.


A \emph{theory} $\mathcal{T}$ over a vocabulary $\Sigma$ is a set that consists of sentences with symbols in $\Sigma$ and  \emph{inductive definitions}. %The vocabulary of a theory $\mathcal{T}$ is denoted $voc(\mathcal{T})$. %A term $t$ containing occurrences of a term $t^\prime$ is denoted as $t[t^\prime]$; the replacement of $t^\prime$ in $t$ by $t^{\prime\prime}$ is denoted as $t[t^\prime / t^{\prime \prime}]$ (similarly for formulas).


An \emph{inductive definition} $\Delta$ is a set of rules of the form: $\forall \overline{x}:P(\overline{x}) \leftarrow \varphi(\overline{y})$ where $\overline{y} \subset \overline{x}$ and $\varphi(\overline{y})$ is a \fo formula.
We call predicate $P$ the \emph{defined predicate}, or the \emph{head} of the definition. Any other predicate or function symbol in $\Delta$ is called a parameter.


A partial structure over a vocabulary $\Sigma$ is a tuple $(D_{T_1}, \ldots, D_{T_n}, \mathcal{I})$, where for each type $T_i$ of $\Sigma$, the domain $D_{T_i}$ of type $T_i$ is a finite set and $\mathcal{I}$ is a partial $\Sigma$-interpretation. A partial $\Sigma$-interpretation $\mathcal{I}$ is a function mapping the symbols in $\Sigma$; we use $s^{\mathcal{I}}$ to refer to the interpretation of a symbol $s$ in $\mathcal{I}$. An interpretation of a predicate symbol $P/n$ consists of two subsets of $D^n$, denoted as $P^\mathcal{I}_{ct}$ and $P^\mathcal{I}_{cf}$ such that $P^\mathcal{I}_{ct}$ and $P^\mathcal{I}_{cf}$ are disjoint; a partial interpretation for a function symbol $f/n$ is a mapping from a subset of $D^n$ to $D$. %If $f(\bar{d})^\mathcal{I} = \emptyset$, we say the image is \emph{undefined}. %The interpretation of a term with a direct sub-term that is undefined is also undefined; that of an atom with a direct sub-term that is undefined is false. Motivation for these choices is given in the next section.
%The interpretation $\{P^\mathcal{I}_ct, P^\mathcal{I}_cf \}$ of a predicate symbol $P$ is consistent if $P^\mathcal{I}_ct$ and $P^\mathcal{I}_cf$ are disjoint. The interpretation of a partial function is always consistent; that of a (total) function is consistent when no tuple has the empty set as image. A $\Sigma$-interpretation is consistent if the interpretations of all its symbols are consistent.
The interpretation of terms $t^{\mathcal{I}}$ and the satisfaction relation for total structures $S \models \varphi$ are defined as usual. 

%By abuse of notation, we will often identify a structure with its $\Sigma$-interpretation if the domain is clear from the context.
We say a structure $S$ is a \emph{total} structure if the $\Sigma$-interpretation is total. In other words, all the symbols, predicates and functions are defined in the $\Sigma$-interpretation.

%The structures can be order lexicographically in the usual way.
A set of structures can be totally ordered in lexicographical way.

%\begin{itemize}
%\item A \emph{vocabulary} $\Sigma$ consists of a set of types and a set of predicate- and function symbols, annotated with the types of their arguments.
%\item A \emph{structure} $S$ over a vocabulary $\Sigma$ consists of a domain $D_T$, for every type $T$ and an interpretation for a subset of the other elements of $\Sigma$.
%\item A \emph{theory}  $\mathcal{T}$ over a vocabulary $\Sigma$ consists of a set of FO sentences and a set of \emph{inductive definitions}.
%\end{itemize}

%We briefly introduce the concept of \emph{inductive definitions}.
%
%Inductive definitions $\Delta$ are sets of rules of the form $\forall \overline{x}:P(\overline{x}) \leftarrow \varphi(\overline{y})$, with $\overline{y} \subset \overline{x}$ and $\varphi(\overline{y})$ a \fodotidp formula.
%We call predicate $P$ the defined predicate, or the head of the definition.
%Any other predicate or function symbol in $\Delta$ is called a parameter.

Inductive definitions are essentially logic programs in which clause bodies can contain arbitrary first-order formulas. The combination of the declarative specification and the imperative programming environment makes this logic programming tool suitable for solving a large variety of different problems.
The semantics used for the inductive definitions are the well-founded semantics \cite{GelderRS91}. As argued in \cite{tocl/DeneckerT08} this captures the intended meaning of all common forms of definitions  and extends the least model semantics of Prolog for negations. A structure $S$ satisfies $\Delta$ if the interpretation of a defined predicate $P$ in the well-founded model of $S$, constructed relative to the restriction of $S$ to the parameters of $\Delta$ is exactly the relation $P^{S}$.
%Another extension in \fodotidp are the aggregates, these are functions over a set of domain elements, which map such a set to the sum, minimum, maximum, cardinality or product of the elements in that set.

%
%
%A special property of the \fodot family of languages is that they are a ``true'' declarative logic. They can be used to create a specification of knowledge, not to formulate the description of a problem. Hence, it has no operational semantics and has no unique form of inference. This however does not mean we have no interest in solving problems with these logics. On the contrary, the disengagement of knowledge from problem solving and inferences makes that a specification of domain knowledge may be reused for solving multiple tasks and  problems \cite{iclp/DeneckerV08}.
%This leads to the idea of \idp, a knowledge base system, that manages a specification, and provides multiple inferences on it, in order to solve a whole range of problems using a single logic specification.
%
%
%\subsection{The knowledge base system : \idp}
%
%
%We define a knowledge base system (KBS) as a system that supports multiple inferences that can be used on a single specification to be able to execute a range of tasks.
%The \idp (\emph{Imperative Declarative Programming}) framework is such a KBS, it combines a declarative specification
%\footnote{We use \idp syntax in the examples throughout the paper.
%%TODO: OR-operator does not look right in the PDF.
%  Each \idp operator has an associated logical operator, the main (non-obvious) operators being: \code{\&}($\land$), \code{|}($\lor$), $\sim$($\lnot$), \code{!}($\forall$), \code{?}($\exists$), $<=>$($\equiv$), $\sim$\code{=}($\neq$).
%}
%, in \fodotidp, a set of inferences and an imperative manipulation of the specification via the Lua \cite{SPE/IerusalimschyFC96} imperative programming environment \cite{inap/DePooterWD11}.
%We will focus only on the most important inferences, for others and more details, we refer to \cite{WarrenBook/DeCatBBD14}.
%\begin{description}
%\item[Modelchecking] Given a structure $I$, a theory $T$, modelchecking outputs true iff $I\models T$
% \item[Model expansion (mx)] Given a vocabulary $V$, a \fodot theory $T$, and a three-valued structure $I$, that contains a domain $D_T$ for every type in $T$, model expansion outputs two-valued structures $I'$ such that every $I'\models T$.
% \item[Propagation] Given a \fodot theory $T$ and a three-valued structure $I$, propagation returns a new three-valued structure $I'$ such that $I'$ approximates every model of $T$ and is more precise then $I$.
% \item[Deduction] Given a \fodot theory $T$ and a FO sentence $\varphi$, deduction outputs true iff $T\models \varphi$. Note: this method is sound but incomplete.
%\item[Progression]
% In~\cite{iclp/BogaertsTemp}, LTC-theories (Linear Time Calculus) are proposed, a syntactic subclass of \fodot theories that allow to naturally model dynamic systems.
% Given an LTC theory and a structure $I_n$ that provides information about the state of the system on a time point $n$, the \emph{progression} inference can be used to compute the state (or the possible states) at time point n+1 as a new structure $I_{n+1}$.
%Repeating the process, we can compute all subsequent states, effectively simulating the dynamic system defined by T.
% An LTC-theory consists of 3 types of constraints: constraints about the initial situation ($P(0)$), invariants $(\forall t: P(t) \lor Q(t))$, and "bistate" formula's that relates the state on the current point in time with that of the next $(\forall t: P(t) \Rightarrow P(t+1))$.
%\ignore{ A small example is included in listing \ref{progress}, which also contains structure $I_1$ the result of the progression.
%\end{description}
% The imperative programming environment supports a rich set of operators and inferences to take the logical building blocks in an \fodotidp specification (vocabularies, theories, terms and structures) and use these to manipulate them and solve more complex reasoning tasks.
%
% The efficiency of the \idp framework in solving problems has been proved in different settings, like for example the most recent ASP-competitions~(\cite{ASP-Comp-2},~\cite{ASP-Comp-3},~\cite{conf/lpnmr/Alviano}) and in applications (~\cite{corr/Blockeel13}, ~\cite{iclp/VanHertum13}). Also the different parts of the system have proved their use in multiple situations: the search algorithm \minisatid has been demonstrated in~\cite{misc/amadini2013}, where it turned out to be the single-best solver in their MiniZinc portfolio, and in the latest MiniZinc challenges~\cite{url:MinizincChallenge2012}. Next to this \idp is used as a didactic tool in various logic-oriented courses, at KU Leuven and at the University of Luxembourg, among others because of its close adherence to \FO and its support for deduction.
%
%
%We look at a specific small example, the connected graph problem (Listing~\ref{mincolor}), given a graph, we want to know if it is fully connected.
%In our vocabulary, we have a type node (the domain of nodes in the graph), a predicate \texttt{edge(node,node)} (there is an edge between these two nodes) and a predicate \texttt{reaches(node,node)} (this expresses the reachability relation between two nodes).
%The theory contains our definitions and constraints.
%We have one (inductive) definition in this theory, which defines reaches (definitions are given between ``\{'' and ``\}'').
%Next to this, the theory contains 1 constraint: Every 2 nodes should be reachable from one another.
%
%Besides these 3 logical building blocks, we also have the procedural Lua part.
%In this code the solver is called to check a model and print out if the graph is fully connected or not.
%

%Note that the concept of inductive definitions is essential to express what reachable means.
%They capture the construction of the reachability relation.
%First we take all edges: if there is an edge from node $x$ to node $y$, then $y$ is reachable from $x$.
%When we have added all the edges to $reaches$, we start using these to recursively add new tuples to our relation.%: every pair $(x,y)$ where there exists a node $z$ such that $z$ is reachable from $x$ and $y$ is reachable from $z$, must be added to $reaches$.
%If we would try to capture this without definitions, we would soon notice that this is impossible. Say we use the material implication to model the reaches relation:  \\[-25pt]
%\begin{align*}
%& reaches(x,y) \Leftarrow edge(x,y).\\
%& reaches(x,y) \Leftarrow \exists z : reaches(x,z) \land reaches(z,y).
%\end{align*}
%The relation $edge$ can now be empty even though every pair of nodes is in $reaches$. If we use an equivalence, we get following formulation: \\[-15pt]
%\begin{align*}
%& reaches(x,y) \Leftrightarrow edge(x,y)  \lor \exists z :reaches(x,z) \land reaches(z,y).
%\end{align*}
%Still we can have a model in which $edge$ is empty and every possible tuple $(x,y)\in reaches^I$.%reaches This is also not the intended meaning of $reaches$.

\begin{definition} For a structure $S$ and a set $A$ of atoms. We define $S[A]$ to be the set of literals in $S$ for the atoms in the set $A$. Formally:\\
$S[A] := \{P(t_1, \ldots t_n): P(t_1, \ldots t_n) \in A \text{~and~} (t_1^S, \ldots t_n^S) \in P^S_{ct}\} \cup \{P(t_1, \ldots t_n): P(t_1, \ldots t_n) \in A \text{~and~} (t_1^S, \ldots t_n^S) \in P^S_{cf}\}$
\end{definition}


\begin{definition} Let $S$ be a partial structure and $\mathcal{T}$ a theory. We say $S$ is a \emph{partial model} for $\mathcal{T}$ if and only if there exists a total structure $S^\prime \supseteq S$ such that $S^\prime \models T$.
\end{definition}

\begin{definition} Let $S$ be a partial structure, $S^\prime$ be a total structure and $\mathcal{T}$ a theory. We say $S^\prime$ \emph{expands} $S$ for a theory $\mathcal{T}$ if and only if $S^\prime \supset S$ and $S^\prime \models T$.
\end{definition}

\begin{definition} Let $S$ be a partial structure, $S^\prime$ be a total structure and $\mathcal{T}$ a theory. We define $modelexpand(\mathcal{T},S)$ to be the set of all total structures $S^\prime$ such that $S^\prime$ expands $S$ for theory $\mathcal{T}$.
\end{definition}

%If the input structure, now interpreting all types, is inconsistent, this should preferably be detected as soon as possible. This can happen for a number of reasons, such as

\begin{definition} Let $S$ be a total structure, $S^\prime$ be a partial structure and $\mathcal{T}$ a theory such that $S \not \models \mathcal{T}$. We define $min\_incons\_set(\mathcal{T},S)$ as the set of minimal (under set inclusion) partial structure $S^\prime \subseteq S$ such that the theory $\mathcal{T}$ has no models that expand $S$. We define $min\_incons(\mathcal{T},S)$ to be the lexicographically first structure in $min\_incons\_set(\mathcal{T},S)$.
\end{definition}


The IDP system supports a range of functionalities to solve various inference and other logic-related tasks such as model expansion and support for minimal inconsistent sets.

\begin{definition} Let $R$ be a set of atoms and let $S$ be a partial structure consisting on a domain $D$ and interpretation $\mathcal{I}$. We write $\left. S \right|_{R}$ for the restriction of $S$ containing only information about $R$. Formally, $\left. S \right|_{R}:= (D, \left. \mathcal{I} \right|_{R})$, where $s^{\left. \mathcal{I} \right|_{R}} = s$ if $s$ is not a predicate symbol, and $P^{\left. \mathcal{I} \right|_{R}}_{ct} = P^{\mathcal{I}}_{ct} \cap \{(d_1, \ldots, d_n) \in D^n : \text{~for some terms~} t_1, \ldots, t_n, P(t_1, \ldots, t_n) \in R \text{~and~} t^{\mathcal{I}} = d_i \text{~for~} 1 \le i \le n\}$. Similarly for $P^{\left. \mathcal{I} \right|_{R}}_{cf}$ for any $n-$ary predicate symbol $P$.
\end{definition}









\section{The Query Mechanism}\label{sec:query}


The language of \foid was briefly defined in Section \ref{sec:IDP}. In our application specific domain we extend the \foid language.% into \lang.
The vocabulary $\Sigma_{\DACL}^{\fo}$
%language \lang
contains two additional sorts (types), the sort \verb=formula= that refers to the language objects from \DACL and the sort \verb=agent= that refers to the principals in our system.
%The vocabulary $\Sigma_{\DACL}^{\fo}$ associated to the language \lang
$\Sigma_{\DACL}^{\fo}$ contains the standard definitions and symbols of \fo plus the following constants, functions and predicates:
\begin{itemize} \setlength\itemsep{0em}
  \item Constants: $c_p$ for every propositional variable $p$ of \DACL.
  \item Partial functions:
    \begin{itemize}
      \item $\verb=NOT=: \verb=formula= \to \verb=formula=$.
      \item A partial function $\verb=AND=: \verb=formula= \times \verb=formula= \to \verb=formula=$.
      \item A partial function $\verb=SAYS=: \verb=agent= \times \verb=formula= \to \verb=formula=$.
    \end{itemize}
  \item Predicates:
    \begin{itemize}
      \item $\verb=eval(formula)= $: interpretation predicate for \DACL formulas.
      %\item $\verb=says(agnt,form)=$: predicate representing the modality.
      \item $q$ : predicate representing the value of a query.
    \end{itemize}
\end{itemize}



\subsubsection{Translation Mechanism.}


In order to implement a query mechanism for \DACL in IDP we need to translate \DACL theories to \foid theories. For this purpose, we first implement a translation mechanism from \DACL formulae to first-order terms. The formulae of \DACL are reified.\footnote{Reification is the process thought which an abstract concept is turned into an explicit object created in the target language.}

\begin{definition}The translation function $t$ from modal propositional formulae to first-order terms is inductively defined as follows:
\begin{itemize}
  \item $t(p) := c_p$, for every propositional letter $p$.
  \item $t(\neg \varphi) := \verb=NOT(=t(\varphi)\verb=)=$.
  \item $t(\varphi \land \psi) := \verb=AND(=t(\varphi),t(\psi)\verb=)=$.
  \item $t(A ~\says~ \varphi) := \verb=SAYS(=A,t(\varphi)\verb=)=$.

\end{itemize}
\end{definition}

%We implement these using a set of (partial) functions $f_i : terms \mapsto boolean $; $f_i \subseteq \{\verb=neg,and,or,impl=\}$.
%
%
%\begin{verbatim}
%    partial neg(_form): _form
%    partial and(_form,_form): _form
%    partial or(_form,_form): _form
%    partial impl(_form,_form): _form
%%    partial SAYS(IP,Port,_form): _form
%\end{verbatim}

\begin{definition}We call a $\Sigma_{\DACL}^{\fo}$-\emph{structure} $S = (D_{\tiny \verb=formula=},D_{\tiny \verb=agent=}, \mathcal{I})$ \emph{proper} if $D_{\tiny \verb=agent=}$ is the set of all \DACL agents, the elements of $D_{\tiny \verb=formula=}$ are \DACL formulas, $D_{\tiny \verb=formula=}$ is closed under the sub-formula property, and for every $\varphi \in D_{\tiny \verb=formula=}$:
\begin{itemize}
  \item if $\varphi = \neg \psi$, then  $\verb=NOT=^{\mathcal{I}}\verb=(=\neg \psi\verb=)=  = \varphi$.
  \item if $\varphi = \chi \land \psi$, then $\verb=AND=^\mathcal{I}\verb=(=\chi,\psi\verb=)= = \varphi$.
  \item if $\varphi = A ~\says~ \psi$, then  $\verb=SAYS=^\mathcal{I}\verb=(=A,\psi\verb=)= = \varphi$.

\end{itemize}
\end{definition}



Given a \DACL theory $T$, an interpretation predicate \verb=eval= for $T$ evaluates the truth value of \DACL formulae.

%to rewrite \DACL theories we use .... then we need an evaluation procedure (predicate) to get the valueeee
%To evaluate the translated propositional modal formulas into first order terms, we define an evaluation predicate \verb=eval=. \\


\begin{definition}[$\tau$ translation] The translation function $\tau$ from \DACL theories to FO(ID) is inductively defined as follows:
\begin{itemize}
  \item $\tau(\varphi):= \varphi$%For a theory $T =  \varphi $, define $\tau(T) :=  \verb=eval(=t(\varphi)\verb=)= $
  \item $\tau(T \cup \{\varphi\}):= \tau(T) \cup \tau(\varphi)$%For a theory $T =  T_0, \varphi $ define $\tau(T) := \tau(T_0), \verb=eval(=t(\varphi)\verb=)= $
  \item $\tau(T \cup \{\{p_1 \leftarrow \varphi_1, \ldots, p_n \leftarrow \varphi_n \ \}\}):= \tau(T) \cup \{\{\verb=eval(=p_1\verb=)= \leftarrow \verb=eval(=\varphi_1\verb=)=, \ldots, \verb=eval(=p_n\verb=)= \leftarrow \verb=eval(=\varphi_n\verb=)= \ \}\}$%For a theory $T = T_0, \{ p \leftarrow \varphi\}$ define $\tau(T) := \tau(T_0), \{ \verb=eval(= p\verb=)= \leftarrow \verb=eval(=t(\varphi)\verb=)= \}$
\end{itemize}

We write $\mathcal{T}$ for the theory $T$ after the translation, $\mathcal{T} = \tau(T)$
\end{definition}


In our current setting the structures are composed of finite domains for each type. We assume that the set of agents is finite, the formulas of \DACL are infinite. To represent the \DACL reified formulae in a structure, we define a finite subset. In order to ensure that this finite subset represents the formulae used in the theory, we introduce the notion of \emph{appropriate structure} for a theory.

%-Explain why we work with structures where domain represents a set of \DACL formulae, but that in the implementation we have to work with finite structures so a structure can not represent all \DACL formulae.
%In order to ensure it represents enough formulae, we introduce the notion of ``appropriate structure'' .


\begin{definition} A (partial) structure $S = (D_{\tiny \verb=formula=},D_{\tiny \verb=agent=}, \mathcal{I})$ is \appropriate for a theory $T$ if $S$ is a proper \DACL structure and $D_{\tiny \verb=formula=}$ contains all the formulae occurring in $T$.
\end{definition}


Given a theory $\mathcal{T}$ we can always construct the \appropriate structure $S$, being the sub-formulae closure for all the symbols used as terms in the interpretation predicate \verb=eval=.


%-Note: the ``real'' information (facts about the access control policies) is encoded in the theory itself, thus, the appropriate structure \emph{only} contains all the terms/formulae that appear in \verb=eval(.)=.


%The evaluation predicate mimics the standard sematic definitions of the underlying modal based says logic.
%
% \begin{itemize}
%  \item \verb=eval(P).= for every propositional variable.
%  \item \verb=eval(neg(P))= $\leftarrow \neg$\verb=eval(P).=
%  \item \verb=eval(and(P,Q))= $\leftarrow$  \verb=eval(P) & eval(Q).=
%  \item \verb=eval(or(P,Q))= $\leftarrow$  \verb=eval(P)= $\mid$ \verb=eval(Q).=
%  \item \verb=eval(impl(P,Q))= $\leftarrow \neg$ \verb=eval(P)= $\mid$ \verb=eval(Q).=
%  \item \verb=eval(SAYS(T,P))= $\leftarrow$  \verb=says(T,P).=
%\end{itemize}



\subsubsection{Query Procedure.}

We use the says modality to access the information contained in theories belonging to other principals.  Consider the following example:

\begin{minipage}[t]{0.40\linewidth}
\[ T_A = \left\{
\begin{split}
   &  p \leftarrow r \land T_B ~says~ s.  \\
   &  r.
\end{split}
 \right\} \]
\end{minipage}\hfill
\begin{minipage}[t]{0.40\linewidth}
\[ T_B = \left\{
\begin{split}
   &  s.  \\
   &  p \leftarrow \neg s \land T_A ~says~ p.
\end{split}
 \right\} \]
\end{minipage}
~\\
~\\

In both theories we have a guard, namely, $s$ for theory $T_B$ and $r$ for theory $T_A$. The guards can be checked in the local theory before performing a remote query to other theories. For theory $T_A$ since the guard is true we can continue with the evaluation, but for theory $T_B$, we do not need to perform the remote query since it will always fail because the guard is not true in the theory.


More complex behaviors rather than guards can occur in our theories. Thus, it is important to minimize the amount of remote queries to those which are only relevant.



\begin{definition} We define $A^{\says}$ to be the set of $\Sigma^{\fo}_{\DACL}$ atoms of the form $\verb=eval(SAYS(=t_1,t_2\verb=))=$.

%A predicate \verb=says(T,=$\varphi$\verb=)= is defined as a query about the truth value of $\varphi$-term $\varphi$ to the \emph{theory} $T$. \\
%We call says\emph{-atoms} to the \emph{literals} contained in an \says\emph{-predicate}.\\
%Let $A^{says}$ be the set of says atoms.
\end{definition}

%\begin{definition}[says-atom] Any propositional atom (literals) composing an at-formula.
%\end{definition}


Each says-predicate is associated to procedural call that queries the remote theory. The evaluation of these external queries requires communication. Limiting remote queries to only those which are relevant minimizes the communication overload. %This query minimization also strengthen the security of our system. NEED TO KNOW PRINCIPLE ADD REFS AND SOME TEXT.    \\


%These relevant queries also have an expected truth value needed to complete the information in the theory. Consider the following example:
%
%\[T_A = \{ p \leftarrow B \says \neg r. \} \]
%\[T_B =  C \says x \rightarrow r.  \]
%
%In this example, principal $A$ need to query principal $B$ about the truth value of $r$, and $A$ expects $r$ to be \emph{false} for $p$ to be true. In turn, principal $B$ can only assign a \emph{true} truth value to $r$, in the case that principal $C$ supports $x$ (after querying $C$). Thus, a query from $B$ to $C$ does not add any relevant information to the query from $A$ to $B$.
%
%We take in account this expected value and add it as a parameter for the remote call. Encoding this information reduces the search space and minimizes further remote calls.

The intuition behind this query mechanism is to be able to identify the minimal set of $A^{\says}$ atoms necessary for a successful query.


%Either there is a model that supports the query or there is not.


%The procedure to obtain this minimal set of relevant queries can be summarized as follows:
%
%
%\begin{itemize}
%  \item Given a query $\mathcal{Q}$ asked to theory $\mathcal{T}$, and an \appropriate structure $S$ such that $S \models \mathcal{T}$. We generate a new theory $\mathcal{T}^\prime$ by adding an inductive definition for the query $\mathcal{Q}$, as follows, $\mathcal{T}^\prime = \mathcal{T}, \{q \leftarrow \mathcal{Q}\}$ for a \emph{new} introduced propositional variable $q$ that will represent the value of the query.
%%      \[ \mathcal{T}_1^\prime = \left\{
%%            \begin{split}
%%            &  \mathcal{T}_1, \{q \leftarrow \mathcal{Q}\} \text{ if } \upsilon = true   \\
%%            &  \mathcal{T}_1, \{q \leftarrow \neg \mathcal{Q}\} \text{ if } \upsilon = false
%%            \end{split}
%%        \right. \]
%%      for a new introduced propositional variable $q$ that will represent the value of the query.
%  \item We expand the models for theory $\mathcal{T}^\prime$ to generate a set of structures $\mathcal{S}$ such that $S \subseteq S^\prime$ for every structure $S^\prime \in \mathcal{S}$ and $S^\prime \models \mathcal{T}^\prime$.
%  \item For every structure $S^\prime \models q$, let $S^s$ be a structure where we switch the truth value of $q$ to false such that $S^s \not \models q$.
%%%      in $S_i^\prime$ i.e.:
%%%        \[ S_i^s = \left\{
%%%            \begin{split}
%%%            &  q := false \text{ if } S_i^\prime \models q   \\
%%%            &  q := true \text{ if } S_i^\prime \not \models q
%%%            \end{split}
%%%        \right. \]
%
%    %$S3 := S2[q: \| \neg q \|_{S2}]$.
%    By construction of the structures $S^s$ we have $S^s \not \models \mathcal{T}^\prime$. We have that $S^\prime \models \mathcal{Q}$ and since $\mathcal{Q}$ does not contain $q$, then $S^s \models \mathcal{Q}$ but $S^s \not \models q$. Thus, $S^s$ can not model the theory $\mathcal{T}^\prime$ considering that $\{q \leftarrow \mathcal{Q}\} \in \mathcal{T}^\prime$.
%
%  \item Finally we compute the minimal set $A$ of says-atoms such that $\left. S^s \right|_{A^{\says} \cup q}  \not \models \mathcal{T}^\prime$. %Furthermore, there is no other structure $S_4$ such that $\left. S_3 \right|_{A \cup q} \subseteq S_4$ and $S_4 \models T_1^\prime$.
%\end{itemize}



\begin{algorithm*}[h!t]
\caption{\textsf{Query Procedure} \label{alg:query}}
\begin{algorithmic}[1]
\REQUIRE{\scriptsize $T$, $\mathcal{Q}$}
\ENSURE{\scriptsize $\mathcal{A}$}
    \STATE{$\mathcal{A}$ := $\emptyset$ }
    \STATE{construct appropriate $S$ for $T$}
    \STATE{$\mathcal{T}^\prime$ := $\tau(T) \cup \{q \leftarrow \verb=eval(=\tau(\mathcal{Q})\verb=)=\}$ }
\STATE{models := modelexpand($\mathcal{T}^\prime$, $S$)}
\FOR{ \textbf{each} $S^\prime = (D_{formula}, D_{agent}, \mathcal{I}) \in $ models}
      \STATE{$S^s := S^\prime$}
      \IF{$S^\prime \models q$}
        \STATE{$\mathcal{I}^s := \mathcal{I}$}
        \STATE{$\mathcal{I}^s(q)$ := \textbf{false} }
        \STATE{$S^s$ := $(D_{formula}, D_{agent}, \mathcal{I}^s)$}
        \IF{$\left. S^s \right|_{A^{\says} \cup q} \models \mathcal{T}^\prime$}\STATE{\textbf{break}} \ENDIF
        \STATE{$S_{min}$ := min\_incons($\mathcal{T^\prime}$, $\left. S^s \right|_{A^{\says} \cup q} $)}
        \STATE{ $\mathcal{A}$ := $\mathcal{A} \cup S_{min}[A^{says}]$}\label{lin:last}
    \ENDIF
\ENDFOR
\RETURN{$\mathcal{A}$}
\end{algorithmic}
\end{algorithm*}
~

The algorithm is to be read as follows. First, given a query $\mathcal{Q}$ asked to theory $\mathcal{T}$, and an \appropriate structure $S$ such that $S \models \mathcal{T}$, we first augment the theory $\mathcal(T)$ adding the inductive definition $\{q \leftarrow \mathcal{Q}\}$ for a \emph{new} introduced propositional variable $q$ that will represent the value of the query.
As second step, we expand the structure $S$ for the augmented theory $\mathcal{T}^\prime$. This generates a set \texttt{models} of structures $\mathcal{S}$ such that $S \subseteq S^\prime$ for every structure $S^\prime \in \mathcal{S}$ and $S^\prime \models \mathcal{T}^\prime$.
From this set of structures $\mathcal{S}$, select those which satisfy the query, namely some structure $S^\prime$ where the (new) propositional variable $q$ representing the query is true.
We iterate over this set for all selected structures. For every structure $S^\prime \models q$, we define $S^s$ to be the structure that makes $q$ false and agrees with $S^\prime$ on every other symbol but $q$. %switch the truth value of $q$ to false such that $S^\prime \not \models q$. Thus making the structure $^\prime$ inconsistent respect with the augmented theory i.e. not a model. This is guaranteed by construction. Lets now call the new structure $S^s$ and the original $S^\prime$ to avoid confusion.
We have that $S^\prime \models \mathcal{Q}$. Since $\mathcal{Q}$ does not contain $q$ it follows $S^s \models \mathcal{Q}$. But since $S^s \not \models q$, $S^s$ can not model the theory $\mathcal{T}^\prime$ considering that $\{q \leftarrow \mathcal{Q}\} \in \mathcal{T}^\prime$.
In step 6, we use the function $min\_incons$ to compute the minimal structure $S_{min}$ such that $S_{min} \subseteq S^\prime$ and $S_{min} \not \models \mathcal{T}^\prime$.
As we will prove later in Theorem \ref{thm:thm1} $S_{min}$ contains the set of \says~ literals that fix the truth value of the query to be true.
%Since we input of the function is the restricted structure $\left. S^\prime \right|_{A^{\says} \cup q}$ that contains only information about the $\says$ predicate and the variable $Q$, the output structure $S^u$ contains the set of \says-atoms that will fix the truth value of the query.
Finally (line \ref{lin:last}) we collect in a set the minimal sets of \says literals that fix the truth value of the query. As last step we return the value of this set.


\begin{lemma}Let $\mathcal{T}^\prime$ be as defined in Algorithm \ref{alg:query}. For every minimal set $A$ making $\mathcal{Q}$ true, there is a structure $S$ such that $S \models A$ and $A$ is the only minimal set such that $A \cup \{\neg q\} \cup \mathcal{T}^\prime$ is inconsistent.

%We know that $unsatstructure(\mathcal{T}^\prime,S[q::f]\mid_{A^{\says} \cup \{q\}})=A$
\end{lemma}

\begin{definition} Let $\mathcal{T}$ be an \foid theory, let $S$ be a partial structure, let $A$ be a set of \foid formulae and let $\varphi$ be an \foid formula. We say that $A$ \emph{fixes} the truth value of $\varphi$ to be true relative to $\mathcal{T}$ and $S$ if and only if for every total structure $S^\prime \supseteq S$ such that $S^\prime \models \mathcal{T}$ and $s^\prime \models A$, we have $S^\prime \models \varphi$.
\end{definition}


\begin{theorem}\label{thm:thm1} Let $\mathcal{T}$ be an \foid theory, let $S$ be a partial structure. The set $\mathcal{A}$ obtained by Algorithm \ref{alg:query} is the set of all $A$ that satisfy the following two properties:
\begin{itemize}  %- For every $A \in \mathcal{A}$ \\ %satisfies the following two properties:
        \item $A$ fixes the truth value of $q$ to be true relative to $\mathcal{T}$ and $S$.
        \item $A$ is a minimal (under set inclusion) set that defines the truth value of $q$ to be true relative to $\mathcal{T}$ and $S$.
\end{itemize}
  %- the set $\mathcal{A}$ contains all sets $A$ satisfying properties 1 and 2.
\end{theorem}




%\subsubsection{General Overview and Intuition.}
%
%
%Given a set of principals $P_1, \ldots, P_n$ each principal has an associated theory (knowledge base) $T_1, \ldots, T_n$ responsible of reasoning about the authorizations granted. Any theory can access the information in other theories (that have to be referenced by name in a peer2peer fashion) using a special predicate \says. The \says-predicates are used to connect different theories (this can be seen an external predicate [Valerio]).
%
%
%Suppose some query $\mathcal{Q}$ in theory $T_1$ which needs some information contained in theory $T_r$ . We generate a partial structure satisfying $T_1$. Which is the minimal amount of questions/information (query) we need from $T_r$? We want to limit the amount of communication among the theories and `ask' just the most necessary questions.
%
%The aim is to find a minimal set $A$ of says-atoms such that the truth value of $\mathcal{Q}$ is fixed. Furthermore, all models generated from (expanding) the structure $S \cup A$ that assign the same truth value to $\mathcal{Q}$.


\subsubsection{Example:}


We first start with a motivating example:


\begin{minipage}[t]{0.48\linewidth}
\[ T_A = \left\{
\begin{split}
   &  p \leftarrow r \land T_B \says b.  \\
   &  r.
\end{split}
 \right\} \]
\end{minipage}\hfill
\begin{minipage}[t]{0.48\linewidth}
\[ T_B = \left\{
\begin{split}
   &  s.  \\
   &  p \leftarrow \neg s \land T_A \says p.
\end{split}
 \right\} \]
\end{minipage}



We translate the theories as follows:


\[ \mathcal{T}_A = \left\{
\begin{split}
   &  eval(p) \leftarrow eval(AND(r,SAYS(T_B,s))).  \\
   &  eval(r).
\end{split}
 \right\} \]

\[ \mathcal{T}_B = \left\{
\begin{split}
   &  eval(s).  \\
   &  eval(p) \leftarrow eval(AND(NEG(s),SAYS(T_A,p))).
\end{split}
 \right\} \]

We construct the an \appropriate structure for $\mathcal{T}_A$ 
%\subsection{Architecture/Topology}
%
%
%\input{topology}


\section{Conclusions and Further Work}\label{sec:conc}

Further Work: define formal semantics for \DACL and show that the query procedure corresponds to the proposed semantics.  








